Unusual magnetic phases in the strong interaction limit of two-dimensional topological band insulators in transition metal oxides

The expected phenomenology of non-interacting topological band insulators (TBI) is now largely theoretically understood. However, the fate of TBIs in the presence of interactions remains an active area of research with novel, interaction-driven topological states possible, as well as new exotic magnetic states. In this work we study the magnetic phases of an exchange Hamiltonian arising in the strong interaction limit of a Hubbard model on the honeycomb lattice whose non-interacting limit is a two-dimensional TBI recently proposed for the layered heavy transition metal oxide compound, (Li,Na)$_2$IrO$_3$. By a combination of analytical methods and exact diagonalization studies on finite size clusters, we map out the magnetic phase diagram of the model. We find that strong spin-orbit coupling can lead to a phase transition from an antiferromagnetic Ne\'el state to a spiral or stripy ordered state. We also discuss the conditions under which a quantum spin liquid may appear in our model, and we compare our results with the different but related Kitaev-Heisenberg-$J_2$-$J_3$ model which has recently been studied in a similar context.

==> Response_to_editor.tex <==

Dear Dr. Ashot Melikyan,

Thank you for your recent correspondence on our manuscript:

Re: BU11954 Kargarian
   Unusual magnetic phases in the strong interaction limit of
    two-dimensional topological band insulators in transition metal oxides
     Mehdi Kargarian, Abdollah Langari, and Gregory A. Fiete


We have revised the Fig.7 and replaced it with new one.  And also we incorporated the "Note added..."  into the main text.


 
Sincerely Yours,
Mehdi Kargarian

List of changes:

1- Fig.7 was revised and replaced with new one. In new figure we plot "1-F" for better look. We added a sentence in Sec.VI to elaborate this change. 

2- We incorporated the paragraph "Note added..." into the main text. We had already cited this work in main text in pages 5 and 6, and now we added a sentence in Sec.VII (Conclusions and Further Remarks) to further incorporate this work.  We also updated its  journal reference in references. 

